Detection of AQM on Paths using Machine Learning Methods

In this paper, we address the problem of determining whether a bottleneck router on a given network path is using an AQM or a drop-tail scheme. We assume that we are given a source-to-sink path of interest -along which a bottleneck router exists- and data regarding the Round-Trip Times (RTT) and Congestion Window (CWND) sizes with respect to this flow. We develop a reliable classification algorithm that solely uses RTT and CWND information pertaining to a single flow to classify the queuing scheme, Tail Drop or AQM, used by the bottleneck router. We evaluate our method and present results that demonstrate our algorithm's highly accurate classification ability across a wide array of complex network topologies and configurations.

==> contributions.tex <==
\section{Contributions}
\emph{Cenk Baykal} developed the algorithm used to generate the random network configurations and helped develop the features that were used to classify the queueing scheme. 
\\

\emph{Wilko Schwarting} worked on the classification algorithm and evaluated state-of-the-art classification methods and conducted hyper-parameter optimization.
\\

\emph{Alex Wallar} developed the Mininet codebase that was used to simulate the randomly generated network configurations and obtain data.

